A Rigorous Study Of The Deep Taylor Decomposition

Saliency methods attempt to explain deep neural networks by highlighting the most salient features of a sample. Some widely used methods are based on a theoretical framework called Deep Taylor Decomposition (DTD), which formalizes the recursive application of the Taylor Theorem to the network's layers. However, recent work has found these methods to be independent of the network's deeper layers and appear to respond only to lower-level image structure. Here, we investigate the DTD theory to better understand this perplexing behavior and found that the Deep Taylor Decomposition is equivalent to the basic gradient$\times$input method when the Taylor root points (an important parameter of the algorithm chosen by the user) are locally constant. If the root points are locally input-dependent, then one can justify any explanation. In this case, the theory is under-constrained. In an empirical evaluation, we find that DTD roots do not lie in the same linear regions as the input - contrary to a fundamental assumption of the Taylor theorem. The theoretical foundations of DTD were cited as a source of reliability for the explanations. However, our findings urge caution in making such claims.

==> relevance_figure.tex <==

\tikzset{>=latex} % for LaTeX arrow head
\colorlet{myred}{red!80!black}
\colorlet{myblue}{blue!80!black}
\colorlet{mygreen}{green!60!black}
\colorlet{myorange}{orange!70!red!60!black}
\colorlet{mydarkred}{red!30!black}
\colorlet{mydarkblue}{blue!40!black}
\colorlet{mydarkgreen}{green!30!black}
\tikzstyle{node}=[thick,circle,draw=myblue,minimum size=22,inner sep=0.5,outer sep=0.6]
\tikzstyle{node in}=[node,green!20!black,draw=mygreen!30!black,fill=mygreen!25]
\tikzstyle{node hidden}=[node,blue!20!black,draw=myblue!30!black,fill=myblue!20]
\tikzstyle{node convol}=[node,orange!20!black,draw=myorange!30!black,fill=myorange!20]
\tikzstyle{node out}=[node,red!20!black,draw=myred!30!black,fill=myred!20]
\tikzstyle{connect}=[thick,mydarkblue] %,line cap=round
\tikzstyle{connect arrow}=[-{Latex[length=4,width=3.5]},thick,mydarkblue,shorten <=0.5,shorten >=1]
\tikzset{ % node styles, numbered for easy mapping with \nstyle
  node 1/.style={node in},
  node 2/.style={node hidden},
  node 3/.style={node out},
}
\def\nstyle{int(\lay<\Nnodlen?min(2,\lay):3)} % map layer number onto 1, 2, or 3



\begin{tikzpicture}[x=2.7cm,y=1.6cm]
    \def\NI{3} % number of nodes in input layers
    \def\NH{4} % number of nodes in input layers
    \def\NO{1} % number of nodes in output layers
    \def\yshift{0.0} % shift last node for dots

    % INPUT LAYER
    \foreach \i [evaluate={
        \c=int(\i==\NI);
        \y=\NI/2-\i-\c*\yshift;
        \index=(\i<\NI?int(\i):"n");
        }]
                in {1,...,\NI}{ % loop over nodes
      \node[node in,outer sep=0.6] (NI-\i) at (0,\y) {$x_{\index}$};
    }

    % HIDDEN LAYER
    \foreach \i [
            evaluate={\c=int(\i==\NH);
            %\y=\NH/2-\i-\c*\yshift;
            \y=0.7*\NH/2-0.7*\i-\c*\yshift;
            \index=(\i<\NH?int(\i):"n");}
        ] in {1,...,\NH}{ % loop over nodes
      \node[node hidden,outer sep=0.3] (NH-\i) at (0.5,\y) {$\vh_{\idx{\index}}$};
      \foreach \j [evaluate={\index=(\j<\NI?int(\j):"n");}] in {1,...,\NI}{ % loop over nodes in previous layer
        \draw[connect,black,line width=0.4] (NI-\j) -- (NH-\i);
        \draw[connect] (NI-\j) -- (NH-\i) node[pos=0.50] {};
      }
    }

    % OUTPUT LAYER
    \foreach \i [evaluate={
        \c=int(\i==\NO);
        \y=\NO/2-\i-\c*\yshift;
        \index=(\i<\NO?int(\i):"m");
    }]
      in {\NO,...,1}{ % loop over nodes
      \ifnum\i=1 % high-lighted node
        \node[node hidden]
          (NO-\i) at (1,\y) {$a_{\index}^{(1)}$};
        \foreach \j [evaluate={\index=(\j<\NI?int(\j):"n");}] in {1,...,\NH}{ % loop over nodes in previous layer
          \draw[connect,white,line width=1.2] (NH-\j) -- (NO-\i);
          \draw[connect] (NH-\j) -- (NO-\i)
            node[pos=0.50] {
               % \contour{white}{$w_{1,\index}$}
            };
        }
      \else % other light-colored nodes
        \node[node,blue!20!black!80,draw=myblue!20,fill=myblue!5]
          (NO-\i) at (1,\y) {$a_{\index}^{(1)}$};
        \foreach \j in {1,...,\NO}{ % loop over nodes in previous layer
          %\draw[connect,white,line width=1.2] (NI-\j) -- (NO-\i);
          \draw[connect,gray!20] (NH-\j) -- (NO-\i);
        }
      \fi
    }
\end{tikzpicture}
